Workload-Aware Monitoring for AI-RAN

AI-RAN platforms are expected to share CPU and GPU resources between radio workloads and AI services. Aggregate telemetry reports operating conditions, but timing changes may reflect different workloads, processors, or measurement boundaries. We propose workload-aware monitoring that associates radio-work descriptors with processing paths, timing boundaries, and operating context before comparing like with like. In 16 over-the-air downlink experiments, hybrid dispatch (CPU for transport blocks (TBs) below 4,096 bytes and GPU otherwise) has 29.66% and 22.93% lower mean host-callback durations than direct GPU dispatch, without and with a synthetic GPU co-runner, respectively. Grouping locates the separation in small TBs, while large-TB callback-duration ranges overlap. These observations identify a candidate for complementary CPU/GPU use.

==> arxiv_notice_conext.tex <==
% This overlays a first-page notice without changing the document flow.
% Coordinates match the supplied US-letter camera-ready PDF.
\RequirePackage{eso-pic}
\AddToShipoutPictureFG*{%
  \AtPageUpperLeft{%
    \begingroup
    \setlength{\unitlength}{1bp}%
    \put(0,-52){%
      \makebox[\paperwidth][c]{%
        \normalfont\fontfamily{ptm}\selectfont\itshape
        \fontsize{9bp}{11bp}\selectfont
        Accepted for publication. To appear in the proceedings of the ACM CoNEXT 2026 Student Workshop.%
      }%
    }%
    \endgroup
  }%
}

